Efficient Consensus-Free Weight Reassignment for Atomic Storage (Extended Version)

Weighted voting is a conventional approach to improving the performance of replicated systems based on commonly-used majority quorum systems in heterogeneous environments. In long-lived systems, a weight reassignment protocol is required to reassign weights over time in order to accommodate performance variations accordingly. The weight reassignment protocol should be consensus-free in asynchronous failure-prone systems because of the impossibility of solving consensus in such systems. This paper presents an efficient consensus-free weight reassignment protocol for atomic storage systems in heterogeneous, dynamic, and asynchronous message-passing systems. An experimental evaluation shows that the proposed protocol improves the performance of atomic read/write storage implemented by majority quorum systems compared with previous solutions.

==> figures/hierarchi.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,101); %set diagram left start at 0, and has height of 101

%Straight Lines [id:da8081000976984176]
\draw    (5.24,15.75) -- (5.19,40.78) ;
%Straight Lines [id:da7552813226704536]
\draw    (5.19,24.4) -- (9.46,24.4) ;
%Straight Lines [id:da9079350771599928]
\draw    (5.19,40.78) -- (9.46,40.78) ;
%Straight Lines [id:da5029404371931037]
\draw    (12.83,47.75) -- (12.83,56.63) ;
%Straight Lines [id:da9472129436689873]
\draw    (13.18,56.63) -- (17.44,56.63) ;
%Straight Lines [id:da813172871945014]
\draw    (22.49,63.81) -- (22.44,88.75) ;
%Straight Lines [id:da29106686553912664]
\draw    (22.88,72.64) -- (27.14,72.64) ;
%Straight Lines [id:da030710770493266315]
\draw    (22.88,88.75) -- (27.14,88.75) ;

% Text Node
\draw (1.37,3.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Majority Quorum Systems};
% Text Node
\draw (9.47,34.62) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Weighted Majority Quorum System};
% Text Node
\draw (9.03,18.84) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Strict Majority Quorum System};
% Text Node
\draw (17.14,51.18) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Dynamic Weighted Majority Quorum System (DWMQS)};
% Text Node
\draw (26.75,66.96) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {DWMQS based on Consensus-based Weight Reassignment};
% Text Node
\draw (27.09,83.31) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {DWMQS based on Consensus-free Weight Reassignment \textit{(this paper)}};


\end{tikzpicture}

